Algorithms for hard-constraint point processes via discretization

We study algorithmic applications of a natural discretization for the hard-sphere model and the Widom-Rowlinson model in a region $\mathbb{V}\subset\mathbb{R}^d$. These models are used in statistical physics to describe mixtures of one or multiple particle types subjected to hard-core interactions. For each type, particles follow a Poisson point process with a type specific activity parameter (fugacity). The Gibbs distribution is characterized by the mixture of these point processes conditioned that no two particles are closer than a type-dependent distance threshold. A key part in better understanding the Gibbs distribution is its normalizing constant, called partition function. We give sufficient conditions that the partition function of a discrete hard-core model on a geometric graph based on a point set $X \subset \mathbb{V}$ closely approximates those of such continuous models. Previously, this was only shown for the hard-sphere model on cubic regions $\mathbb{V}=[0, \ell)^d$ when $X$ is exponential in the volume of the region $\nu(\mathbb{V})$, limiting algorithmic applications. In the same setting, our refined analysis only requires a quadratic number of points, which we argue to be tight. We use our improved discretization results to approximate the partition functions of the hard-sphere model and the Widom-Rowlinson efficiently in $\nu(\mathbb{V})$. For the hard-sphere model, we obtain the first quasi-polynomial deterministic approximation algorithm for the entire fugacity regime for which, so far, only randomized approximations are known. Furthermore, we simplify a recently introduced fully polynomial randomized approximation algorithm. Similarly, we obtain the best known deterministic and randomized approximation bounds for the Widom-Rowlinson model. Moreover, we obtain approximate sampling algorithms for the respective spin systems within the same fugacity regimes.

==> content/non_starconvex.tex <==
%\section{Concentration without star-convexity}
%All results considered so far used the assumption that the region $\volume$ is star-convex.
%This is essentially due to \Cref{lemma:discretization_error:1}, which bounds the error introduced by mapping each point according to an allocation $\allocation$.
%However, it turns out that a slightly weaker version of the concentration results for discretizations based on random point sets, given in \Cref{sec:random_discretization} \todo{change this reference when merging Sec 8 and 9}, also holds without the assumption of star-convexity.
%
%The core idea is to argue that $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$ is not significantly larger than $\allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}$,  instead of arguing that they are close in general as done in \Cref{lemma:discretization_error:1}.
%This argument does not require star-convexity.
%By randomizing the set of points, we obtain sufficient conditions for $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$ to concentrate from below.
%The following general lemma then establishes that the partition function of the hard-core representation also concentrates from above.
%
%\begin{lemma}
%	\label{lemma:modified_markov}
%	Let $\randomVariable$ be a non-negative random variable with finite expectation.
%	If there are $\genericError \in \R_{>0}$ and $\genericFailingProb \in [0, 1]$ such that $\Pr{\randomVariable < (1-\genericError) \E{\randomVariable}} \le \genericFailingProb$, then it holds that $\Pr{\randomVariable \ge (1 + c \genericError) \E{\randomVariable}} \le \frac{1}{c+1} \left(1 + \frac{\genericFailingProb}{\genericError}\right)$ for all $c \in \R_{\ge 0}$.
%\end{lemma}
%
%\begin{proof}
%	Let $A$ denote the event that $\randomVariable \ge (1-\genericError) \E{\randomVariable}$ and set $\modifiedRandomVariable = \ind{A} (\randomVariable - (1 - \genericError) \E{\randomVariable})$.
%	Using the fact that $\randomVariable$ is non-negative and $\Pr{A} \ge 1 - \genericFailingProb$ we obtain\todo{Why do we drop the $-\delta\varepsilon$ already in this theorem?}
%	\begin{align*}
%		\E{\modifiedRandomVariable}
%		&= \E{\ind{A} \randomVariable} - (1 - \genericError) \E{\randomVariable} \Pr{A} \\
%		&\le \E{\randomVariable} - (1 - \genericFailingProb)(1 - \genericError) \E{\randomVariable} \\
%		&= (\genericFailingProb + \genericError - \genericFailingProb \genericError) \E{\randomVariable} \\
%		&\le (\genericFailingProb + \genericError) \E{\randomVariable}.
%	\end{align*}
%	Further, observe that $\modifiedRandomVariable$ is non-negative and that $\randomVariable \ge (1 + c \genericError) \E{\randomVariable}$ if and only if $\modifiedRandomVariable \ge (c+1) \genericError \E{\randomVariable}$.
%	By using Markov's inequality, we get
%	\begin{align*}
%		\Pr{\randomVariable \ge (1 + c \genericError) \E{\randomVariable}}
%		&= \Pr{\modifiedRandomVariable \ge (c+1) \genericError \E{\randomVariable}} \\
%		&\le \frac{\E{\modifiedRandomVariable}}{(c+1) \genericError \E{\randomVariable}} \\
%		&\le \frac{(\genericFailingProb + \genericError) \E{\randomVariable}}{(c+1) \genericError \E{\randomVariable}} \\
%		&= \frac{1}{c+1} \left(1 + \frac{\genericFailingProb}{\genericError}\right) ,
%	\end{align*}
%	which concludes the proof.
%\end{proof}
%
%Next, given a suitable allocation $\allocation$, we show that $\allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}$ is not significantly smaller than $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$.
%
%\begin{lemma}
%	\label{lemma:lower_bound}
%	Let $(\volume, \interactionMatrix, \fugacity)$ be a hard-constraint point process with $\numTypes \in \N_{\ge 1}$ particle types.
%	Further, set $\interactionMatrix_{\max} = \max_{i,j \in [\numTypes]} \{\interactionMatrix[i][j]\}$, and set $\fugacity_{\max} = \max_{i \in [\numTypes]} \fugacity[i]$.
%	Let $\volumeError \in \left[0, 1\right]$ and $\distanceError \in \left[0, \frac{1}{2}\right]$ and let $X \subseteq \volume$ such that there is a $\volumeError$-$\distanceError$-allocation $\allocation$ for $X$.
%	Then
%	\[
%		\sum_{\numParticles \in \N} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}} \left(\generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] - \generalWeight{\interactionMatrix}{\fugacity}[\allocation[\mathbold{x}], \typeOf]\right) \, \text{d} \lebesgue{\dimension \times \numParticles}
%		\le \distanceError \numTypes \fugacity_{\max}^2 \vol{\volume} \vol{\ball{\interactionMatrix_{\max} + 1}} \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} .
%		\qedhere
%	\]
%\end{lemma}
%
%\begin{proof}
%	By definition, we have
%	\begin{align}
%		\notag
%		\sum_{\numParticles \in \N} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}} &\left(\generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] - \generalWeight{\interactionMatrix}{\fugacity}[\allocation[\mathbold{x}], \typeOf]\right) \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		\notag
%		&= \sum_{\numParticles \in \N} \frac{1}{\numParticles!} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]}
%		\left(\prod_{i \in [\numParticles]} \fugacity[\typeOf[i]] \right) \int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		\label{lemma:lower_bound:eq_1}
%		&= \sum_{\numParticles \ge 2} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \frac{1}{\numParticles!}
%		\left(\prod_{i \in [\numParticles]} \fugacity[\typeOf[i]] \right) \int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles}.
%	\end{align}
%	We proceed by bounding
%	\[
%		\int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles}
%	\]
%	from above.
%	Set
%	\[
%		L^{(\interactionMatrix)}_{\typeOf, \allocation} = \left\{ \mathbold{x} \in \volume^{\numParticles} \mid \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] = 1 \text{ and } \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] = 0\right\}
%	\]
%	and observe that
%	\[
%		\int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles}
%		\le \vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}} .
%	\]
%	Now, note that for all $\mathbold{x} = (x_1 \dots, x_{\numParticles}) \in \volume^{\numParticles}$ it holds that $\valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] = 0$ if and only if there are $i, j \in [\numParticles]$ with $i \neq j$ such that $\dist{\allocation[x_i]}{\allocation[x_j]} < \interactionMatrix[\typeOf[i]][\typeOf[j]]$.
%	Let
%	\[
%		L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j) = \left\{ \mathbold{x} \in \volume^{\numParticles} \mid \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] = 1 \text{ and } \dist{\allocation[x_i]}{\allocation[x_j]} < \interactionMatrix[\typeOf[i]][\typeOf[j]]\right\}
%	\]
%	and observe that
%	\[
%		\vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}} \le \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j)} .
%	\]
%	Thus, we obtain
%	\[
%		\int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles}
%		\le \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j)} .
%	\]
%	Next, we upper bound $\vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j)}$ for each $i, j \in [\numParticles]$ with $i < j$.
%	To this end, we first introduce some additional notation.
%	For a finite set $S \subset \N$ and $i \in S$ let $\order{S}[i]$ denote the order of $i$ in $S$.
%	That is, $\order{S}[i]\colon S \to [\size{S}]$ with $\order{S}(i) = \size{\{j \in S \mid j \le i\}}$.
%	Let $\numParticles \ge 2$, $\mathbold{x} = (x_1, \dots, x_{\numParticles}) \in \volume^{\numParticles}$ and $\typeOf\colon [\numParticles] \to [\numTypes]$.
%	For any $S \subseteq [\numParticles]$ let $\mathbold{x}_{-S} \in \volume^{\numParticles - \size{S}}$ denote $\mathbold{x}$ after removing all components index by $S$.
%	Further, define $\typeOf_{-S}: [\numParticles - \size{S}] \to [\numTypes]$ where for each $i \in [\numParticles] \setminus S$ we set $\typeOf_{-S}(\order{[\numParticles] \setminus S}[i]) = \typeOf[i]$.
%	Informally speaking, $\mathbold{x}_{-S}$ and $\typeOf_{-S}$ represent the configuration that results from $\mathbold{x}$ and $\typeOf$ after removing the particles index by the set $S$.
%
%	With this additional notation, we proceed with upper bounding $\vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j)}$.
%	Recall that $\allocation$ is a $\volumeError$-$\distanceError$-allocation, which implies $\dist{x}{\allocation[x]} \le \distanceError$ for all $x \in \volume$.
%	We obtain
%	\begin{align*}
%		\vol{L^{(\interactionMatrix)}_{\typeOf, \allocation}(i, j)}
%		&= \int_{\volume^{\numParticles}}  \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] \ind{\dist{\allocation[x_i]}{\allocation[x_j]} < \interactionMatrix[\typeOf[i]][\typeOf[j]]} \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&\le \int_{\volume^{\numParticles}}  \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}_{-\{i, j\}}] \ind{\dist{x_i}{x_j} \ge \interactionMatrix[\typeOf[i]][\typeOf[j]] \text{ and } \dist{\allocation[x_i]}{\allocation[x_j]} < \interactionMatrix[\typeOf[i]][\typeOf[j]]} \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&\le \int_{\volume^{\numParticles}}  \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}_{-\{i, j\}}] \ind{\interactionMatrix[\typeOf[i]][\typeOf[j]] \le \dist{x_i}{x_j} < \interactionMatrix[\typeOf[i]][\typeOf[j]] + 2\distanceError} \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&\le \left(\vol{\ball{\interactionMatrix[\typeOf[i]][\typeOf[j]] + 2 \distanceError}} - \vol{\ball{\interactionMatrix[\typeOf[i]][\typeOf[j]]}}\right) \vol{\volume} \int_{\volume^{\numParticles-2}}  \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}] \text{d} \lebesgue{\dimension \times (\numParticles-2)} .
%	\end{align*}
%	Further, observe that for $\distanceError \le \frac{1}{2}$ it holds that
%	\begin{align*}
%		\left(\vol{\ball{\interactionMatrix[\typeOf[i]][\typeOf[j]] + 2 \distanceError}} - \vol{\ball{\interactionMatrix[\typeOf[i]][\typeOf[j]]}}\right)
%		&\le \vol{\ball{1}} \left((\interactionMatrix_{\max} + 2 \distanceError)^{\dimension} - \interactionMatrix_{\max}^{\dimension}\right) \\
%		&= \vol{\ball{1}} \sum_{i = 1}^{\dimension} \binom{\dimension}{i} \left(2 \distanceError\right)^{i} \interactionMatrix_{\max}^{\dimension - i} \\
%		&= 2 \distanceError \vol{\ball{1}} \sum_{i = 1}^{\dimension} \binom{\dimension}{i} \left(2 \distanceError\right)^{i-1} \interactionMatrix_{\max}^{\dimension - i} \\
%		&\le 2 \distanceError \vol{\ball{1}} (\interactionMatrix_{\max} + 1)^{\dimension} \\
%		&= 2 \distanceError \vol{\ball{\interactionMatrix_{\max} + 1}}.
%	\end{align*}
%	Thus, we have
%	\begin{align*}
%		\int_{\volume^{\numParticles}} \left( \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] - \valid{\typeOf}{\interactionMatrix}[\allocation[\mathbold{x}]] \right) \, \text{d} \lebesgue{\dimension \times \numParticles}
%		&\le 2 \distanceError \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume}  \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \int_{\volume^{\numParticles-2}}  \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}] \text{d} \lebesgue{\dimension \times (\numParticles-2)} .
%	\end{align*}
%	Substituting this back into \cref{lemma:lower_bound:eq_1} and observing that
%	\begin{align*}
%		2 \distanceError \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \frac{1}{\numParticles!}
%		&\left(\prod_{l \in [\numParticles]} \fugacity[\typeOf[l]] \right) \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \int_{\volume^{\numParticles-2}}  \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}] \text{d} \lebesgue{\dimension \times (\numParticles-2)} \\
%		&= 2 \distanceError \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \int_{\volume^{\numParticles-2}} \frac{1}{\numParticles!}
%		\left(\prod_{l \in [\numParticles]} \fugacity[\typeOf[l]] \right) \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}] \text{d} \lebesgue{\dimension \times (\numParticles-2)} \\
%		&\le 2 \distanceError \frac{\fugacity_{\max}^2}{\numParticles(\numParticles-1)} \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \int_{\volume^{\numParticles-2}} \frac{1}{(\numParticles-2)!}
%		\left(\prod_{\substack{l \in [\numParticles]: \\ l \notin \{i, j\}}} \fugacity[\typeOf[l]] \right) \valid{\typeOf_{-\{i, j\}}}{\interactionMatrix}[\mathbold{x}] \text{d} \lebesgue{\dimension \times (\numParticles-2)} \\
%		&= 2 \distanceError \frac{\fugacity_{\max}^2}{\numParticles(\numParticles-1)} \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \int_{\volume^{\numParticles-2}} \generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf_{-\{i, j\}}] \text{d} \lebesgue{\dimension \times (\numParticles-2)}
%	\end{align*}
%	gives
%	\begin{align*}
%		\sum_{\numParticles \in \N} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}} &\left(\generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] - \generalWeight{\interactionMatrix}{\fugacity}[\allocation[\mathbold{x}], \typeOf]\right) \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&\le 2 \distanceError \frac{\fugacity_{\max}^2}{\numParticles(\numParticles-1)} \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\numParticles \ge 2} \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles-2}} \generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf_{-\{i, j\}}] \text{d} \lebesgue{\dimension \times (\numParticles-2)}  \\
%		&= 2 \distanceError \numTypes^2 \frac{\fugacity_{\max}^2}{\numParticles(\numParticles-1)} \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\numParticles \ge 2} \sum_{\substack{i, j \in [\numParticles]:\\ i<j}} \sum_{\typeOf\colon [\numParticles - 2] \to [\numTypes]} \int_{\volume^{\numParticles-2}} \generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] \text{d} \lebesgue{\dimension \times (\numParticles-2)}  \\
%		&= \distanceError \numTypes^2 \fugacity_{\max}^2 \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\numParticles \ge 2} \sum_{\typeOf\colon [\numParticles - 2] \to [\numTypes]} \int_{\volume^{\numParticles-2}} \generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] \text{d} \lebesgue{\dimension \times (\numParticles-2)} \\
%		&= \distanceError \numTypes^2 \fugacity_{\max}^2 \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume} \sum_{\numParticles \in \N} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}} \generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&= \distanceError \numTypes \fugacity_{\max}^2 \vol{\volume} \vol{\ball{\interactionMatrix_{\max} + 1}} \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} ,
%	\end{align*}
%	which concludes the proof.
%\end{proof}
%
%Combining \Cref{lemma:lower_bound} and \Cref{lemma:discretization_error:2} yields that $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$ also is not much smaller than $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$.
%\begin{lemma}
%	\label{lemma:deterministic_lower_bound}
%	Let $(\volume, \interactionMatrix, \fugacity)$ be a hard-constraint point process with $\numTypes \in \N_{\ge 1}$ particle types.
%	For all $\discretizationError \in \left(0, 1\right]$ there are $\distanceError, \volumeError \in \bigTheta{\discretizationError \vol{\volume}^{-1}}$ such that, for all finite $X \subset \volume$ that have a $\volumeError$-$\distanceError$-allocation and satisfy $\size{X} \ge 64 \numTypes \fugacity_{\max}^2 \vol{\volume}^2 \discretizationError^{-1}$, it holds that
%	\begin{align*}
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge (1 - \discretizationError)\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} ,
%	\end{align*}
%	where $(\hcPPGraph{X}, \hcPPWeight{X})$ is the hard-core representation of $(\volume, \interactionMatrix, \fugacity)$ based on $X$.
%\end{lemma}
%
%\begin{proof}
%	Set $\interactionMatrix_{\max} = \max_{i,j \in [\numTypes]} \interactionMatrix[i][j]$ and $\fugacity_{\max} = \max_{i \in [\numTypes]} \fugacity[i]$.
%	Further, set
%	\[
%		\distanceError
%		= \frac{\discretizationError}{2 \numTypes \fugacity_{\max}^2 \vol{\ball{\interactionMatrix_{\max} + 1}} \vol{\volume}}
%		\in \bigTheta{\discretizationError \vol{\volume}^{-1}}
%	\]
%	and
%	\[
%		\volumeError
%		= \frac{\discretizationError}{16 \numTypes \fugacity_{\max} \vol{\volume}}
%		\in \bigTheta{\discretizationError \vol{\volume}^{-1}} .
%	\]
%	For $\vol{\volume}$ sufficiently large we have $\distanceError \le \frac{1}{2}$ and thus, by \Cref{lemma:lower_bound}, we obtain
%	\begin{align*}
%		\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} - \allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}
%		&= \sum_{\numParticles \in \N} \sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}} \left(\generalWeight{\interactionMatrix}{\fugacity}[\mathbold{x}, \typeOf] - \generalWeight{\interactionMatrix}{\fugacity}[\allocation[\mathbold{x}], \typeOf]\right) \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&\le \frac{\discretizationError}{2} \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity},
%	\end{align*}
%	which implies
%	\begin{align}
%		\label[ineq]{lemma:deterministic_lower_bound:eq1}
%		\allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}\ge \left(1 - \frac{\discretizationError}{2}\right) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} .
%	\end{align}
%
%	Further, note that $\size{X} \ge 64 \numTypes \fugacity_{\max}^2 \vol{\volume}^2 \discretizationError^{-1}  \ge 4 \fugacity_{\max} \vol{\volume}$.
%	Thus, by \Cref{lemma:hcPPPartitionFunction_equivalence,lemma:discretization_error:2}, we have
%	\begin{align*}
%		\absolute{\allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation} - \hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}}
%		&\le \sum_{\numParticles \in \N}
%		\sum_{\typeOf\colon [\numParticles] \to [\numTypes]} \int_{\volume^{\numParticles}}
%		\absolute{\generalWeight{\interactionMatrix}{\fugacity}[\allocation[\mathbold{x}], \typeOf] - \hcPPWeightContinuous{\hcPPGraph{X}}{\hcPPWeight{X}}{\allocation}[\mathbold{x}, \typeOf]} \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%%		&\le \left(\eulerE^{\frac{8}{\size{X}} \sum_{i \in [\numTypes]} \fugacity[i]^2 \vol{\volume}^2} \eulerE^{2 \volumeError \sum_{i \in [\numTypes]} \fugacity[i] \vol{\volume}} - 1\right)	\allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation} \\
%		&\le \left(\eulerE^{\frac{\discretizationError}{4}} - 1\right) \allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}.
%	\end{align*}
%	As $\discretizationError \le 2$ it holds that
%	\begin{align*}
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}
%		&\ge \left(2 - \eulerE^{\frac{\discretizationError}{4}}\right) \allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation}\\
%		&\ge \left(1 - \frac{\discretizationError}{2}\right) \allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation} .
%	\end{align*}
%	Combining this with \cref{lemma:deterministic_lower_bound:eq1} finally gives us
%	\begin{align*}
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}
%		&\ge \left(1 - \frac{\discretizationError}{2}\right) \allocationPartitionFunction{\volume}{\interactionMatrix}{\fugacity}{\allocation} \\
%		&\ge \left(1 - \frac{\discretizationError}{2}\right)^2 \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} \\
%		&\ge (1 - \discretizationError) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} ,
%	\end{align*}
% 	which proves the claim.
%\end{proof}
%
%By randomizing the considered set of points, we turn \Cref{lemma:deterministic_lower_bound} into a bound on how strong $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$ concentrates from below.
%Combining this with \Cref{lemma:modified_markov} then gives two-sided concentration.
%However, note that \Cref{lemma:modified_markov} only works for concentration around the expected value, but \Cref{lemma:deterministic_lower_bound} is given in terms of $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$.
%The following lemma will solves this problem by relating both quantities.
%
%\begin{lemma}
%	\label{lemma:expectation}
%	Let $(\volume, \interactionMatrix, \fugacity)$ be a hard-constraint point process with $\numTypes \in \N_{\ge 1}$ particle types.
%	For all $\numPoints \ge 1$ it holds that
%	\[
%		\E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}} \le \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} ,
%	\]
%	where the expectation is taken over $X \subset \volume$ with $\size{X} = \numPoints$ drawn uniformly at random.
%\end{lemma}
%
%\begin{proof}
%	We start by rewriting $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$ as
%	\begin{align*}
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}
%		= 1 + \sum_{\numParticles = 1}^{\numPoints} \frac{\vol{\volume}^{\numParticles}}{\numPoints^{\numParticles}} \sum_{\substack{(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}: \\ \numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles}} \left(\prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}\right) \sum_{\substack{S_1 \subseteq X:\\ \size{S_1} = \numParticles_1}} \dots \sum_{\substack{S_{\numTypes} \subseteq X:\\ \size{S_\numTypes} = \numParticles_\numTypes}} \ind{\substack{\forall i, j \in [\numTypes] \forall x_1 \in S_i, x_2 \in S_j:\\ (i=j \text{ and } x_1 = x_2)\\ \text{ or } \dist{x_1}{x_2} \ge \interactionMatrix[i][j]}},
%	\end{align*}
%	where the condition $(i=j \text{ and } x_1 = x_2)$ accounts for the fact that $\hcPPGraph{X}$ does not contain self loops.
%	We proceed by rewriting this in terms of tuples of points from $X$.
%	To this end, for every $(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}$ define a canonical type assignment $\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}: [\numParticles_1 + \dots + \numParticles_{\numTypes}] \to [\numTypes]$ with $\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}(i) = j$ such that $\sum_{l=1}^{j-1} \numParticles_l < i \le \sum_{l=1}^{j} \numParticles_l$.
%	For any $\numParticles \in \N$ let $X^{\numParticles}_{\neq} = \{(x_1, \dots, x_{\numParticles}) \mid \forall i, j \in [\numParticles]\colon i \neq j \text{ implies } x_i \neq x_j\}$.
%	Further, for $\mathbold{x} = (x_1, \dots, x_{\numParticles_1}) \in X^{\numParticles_1}$ and $\mathbold{y} = (y_1, \dots, y_{\numParticles_2}) \in X^{\numParticles_2}$ write $\mathbold{x} \concatenation \mathbold{y}$ for the concatenation $(x_1, \dots, x_{\numParticles_1}, y_1, \dots, y_{\numParticles_2}) \in X^{\numParticles_1 + \numParticles_2}$ of both tuples.
%	Observe that
%	\begin{align*}
%		\sum_{\substack{S_1 \subseteq X:\\ \size{S_1} = \numParticles_1}} \dots \sum_{\substack{S_{\numTypes} \subseteq X:\\ \size{S_\numTypes} = \numParticles_\numTypes}} \ind{\forall i, j \in [\numTypes] \forall x_1 \in S_i, x_2 \in S_j: (i=j \text{ and } x_1 = x_2) \text{ or } \dist{x_1}{x_2} \ge \interactionMatrix[i][j]}
%		&= \frac{1}{\numParticles_1 !} \sum_{\mathbold{x_1} \in X^{\numParticles_1}_{\neq}} \dots \frac{1}{\numParticles_{\numTypes} !} \sum_{\mathbold{x_{\numTypes}} \in X^{\numParticles_{\numTypes}}_{\neq}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x_1} \concatenation \dots \concatenation \mathbold{x_{\numTypes}}] \\
%		&\le \left(\prod_{i \in [\numTypes]} \frac{1}{\numParticles_{i}!}\right) \sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}] .
%	\end{align*}
%	Thus, we have
%	\[
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}
%		= 1 + \sum_{\numParticles = 1}^{\numPoints} \frac{\vol{\volume}^{\numParticles}}{\numPoints^{\numParticles}} \sum_{\substack{(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}: \\ \numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles}} \left(\prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}\right) \cdot \left(\prod_{i \in [\numTypes]} \frac{1}{\numParticles_{i}!}\right) \sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}] ,
%	\]
%	which, by monotonicity and linearity of expectation yields
%	\begin{align}
%		\notag
%		\E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}}
%		&\le 1 + \sum_{\numParticles = 1}^{\numPoints} \frac{\vol{\volume}^{\numParticles}}{\numPoints^{\numParticles}} \sum_{\substack{(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}: \\ \numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles}} \left(\prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}\right) \cdot \left(\prod_{i \in [\numTypes]} \frac{1}{\numParticles_{i}!}\right) \E{\sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}]} \\
%		\label[ineq]{lemma:expectation:eq1}
%		&\le 1 + \sum_{\numParticles \in \N_{\ge 1}} \frac{\vol{\volume}^{\numParticles}}{\numPoints^{\numParticles}} \sum_{\substack{(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}: \\ \numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles}} \left(\prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}\right) \cdot \left(\prod_{i \in [\numTypes]} \frac{1}{\numParticles_{i}!}\right) \E{\sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}]}
%	\end{align}
%	Let $x_1, \dots, x_{\numPoints}$ some arbitrary ordering of the points in $X$.
%	Now, note that
%	\[
%		\sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}]
%		= \sum_{(i_1, \dots, i_{\numParticles}) \in [\numPoints]^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[x_{i_1}, \dots, x_{i_{\numParticles}}] .
%	\]
%	Thus, we get
%	\begin{align*}
%		\E{\sum_{\mathbold{x} \in X^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}]}
%		= \sum_{(i_1, \dots, i_{\numParticles}) \in [\numPoints]^{\numParticles}} \E{\valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[x_{i_1}, \dots, x_{i_{\numParticles}}]}
%		= \frac{\numPoints^{\numParticles}}{\vol{\volume}^{\numParticles}} \int_{\volume^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}] \, \text{d} \lebesgue{\dimension \times \numParticles} .
%	\end{align*}
%	Substituting this back into \cref{lemma:expectation:eq1} and canceling some terms yields
%	\[
%		\E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}} \le 1 + \sum_{\numParticles \in \N_{\ge 1}}  \sum_{\substack{(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}: \\ \numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles}} \left(\prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}\right) \cdot \left(\prod_{i \in [\numTypes]} \frac{1}{\numParticles_{i}!}\right)  \int_{\volume^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}] \, \text{d} \lebesgue{\dimension \times \numParticles} .
%	\]
%	Finally, observe that, for each $\numParticles \in \N_{\ge 1}$ and all $(\numParticles_1, \dots, \numParticles_{\numTypes}) \in \N^{\numTypes}$ with $\numParticles_1 + \dots + \numParticles_{\numTypes} = \numParticles$, there a $\frac{\numParticles!}{\prod_{i \in [\numTypes]} \numParticles_{i} !}$ type assignments $\typeOf\colon [\numParticles] \to [\numTypes]$ that are equivalent to $\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}$ up to permutation of inputs (i.e., $\size{\typeOf^{-1} (i)} = \size{\typeOf^{-1}_{\numParticles_1, \dots, \numParticles_{\numTypes}}(i)}$ for each $i \in [\numTypes]$).
%	Further, note that $\prod_{i \in [\numParticles]} \fugacity[\typeOf[i]] = \prod_{i \in [\numTypes]} \fugacity[i]^{\numParticles_i}$ and $\int_{\volume^{\numParticles}} \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] \, \text{d} \lebesgue{\dimension \times \numParticles} = \int_{\volume^{\numParticles}} \valid{\typeOf_{\numParticles_1, \dots, \numParticles_{\numTypes}}}{\interactionMatrix}[\mathbold{x}] \, \text{d} \lebesgue{\dimension \times \numParticles}$ for each such $\typeOf$.
%	Thus, it holds that
%	\begin{align*}
%		\E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}} &\le 1 + \sum_{\numParticles \in \N_{\ge 1}} \frac{1}{\numParticles!}  \sum_{\typeOf: [\numParticles] \to [\numTypes]} \left(\prod_{i \in [\numParticles]} \fugacity[\typeOf[i]]\right)   \int_{\volume^{\numParticles}} \valid{\typeOf}{\interactionMatrix}[\mathbold{x}] \, \text{d} \lebesgue{\dimension \times \numParticles} \\
%		&= \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity},
%	\end{align*}
%	proving the claim.
%\end{proof}
%
%We are now ready to state and prove our main theorem about concentration of random discretizations without star-convexity.
%\begin{theorem}
%	\label{thm:prob_bound_non_starconvex}
%	Let $(\volume, \interactionMatrix, \fugacity)$ be a hard-constraint point process with $\numTypes \in \N_{\ge 1}$ particle types.
%	Further, assume there is some $\volumeScaling \in (0, 1]$ such that for all $\distanceError \in \R_{>0}$ there is a $\volumeScaling$-$\distanceError$-partitioning of $\volume$ of size $\poly{\frac{\vol{\volume}}{\distanceError}}$.
%	For all $\discretizationError \in (0, 1]$ and $\allocationProb \in (0, 1]$ there is some  $\numPoints_{\discretizationError, \allocationProb} \in \poly{\frac{\vol{\volume}}{\discretizationError \allocationProb}}$ such that for all $\numPoints \ge \numPoints_{\discretizationError, \allocationProb}$ it holds for $X \subset \volume$ with $\size{X} = \numPoints$ uniformly at random that
%	\[
%		\eulerE^{-\discretizationError}\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}
%		\le \hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}
%		\le  \eulerE^{\discretizationError}\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}
%	\]
%	with probability at least $1-\allocationProb$.
%\end{theorem}
%
%\begin{proof}
%	The main idea of the proof is to use \Cref{lemma:partitioning_allocation} and \Cref{lemma:deterministic_lower_bound} to argue that, for a uniformly drawn $X \subset \volume$ that is sufficiently large, the hard-core partition function $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$ is with high probability not much smaller than the partition function $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$ of the continuous model.
%	Then we apply \Cref{lemma:modified_markov} to derive a probabilistic upper bound on $\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}$
%
%	Let $c = \frac{\allocationProb}{2}$, $\discretizationError' = \frac{\discretizationError}{c} = \frac{\allocationProb}{2} \discretizationError$ and $\allocationProb' = \frac{\discretizationError}{4} \allocationProb = \frac{\discretizationError'}{2} $.
%	By \Cref{lemma:deterministic_lower_bound}, we know that there are $\distanceError', \volumeError' \in \bigTheta{\discretizationError' \vol{\volume}^{-1}} = \bigTheta{\discretizationError \allocationProb \vol{\volume}^{-1}}$ such that, for all $X \subset \volume$ with $\size{X} \ge 64 \numTypes \fugacity_{\max}^2 \vol{\volume}^2 \discretizationError'^{-1} = 128 \numTypes \fugacity_{\max}^2 \vol{\volume}^2 \discretizationError^{-1} \allocationProb^{-1}$ that have an $\volumeError$-$\distanceError$-allocation, it holds that
%	\[
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge \left(1 - \discretizationError'\right) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} .
%	\]
%
%	Next, note that we assume that there is a $\volumeScaling$-$\distanceError$-partitioning of $\volume$ of size $\poly{\frac{\vol{\volume}}{\distanceError}}$ for some $\volumeScaling \in (0, 1]$ and all $\distanceError \in \R_{>0}$.
%	Thus, by \Cref{lemma:partitioning_allocation} we conclude that there is some \[
%		\numPoints'_{\discretizationError, \allocationProb}
%		\in \poly{\frac{\vol{\volume}}{\distanceError' \volumeError'} \ln\left(\frac{1}{\allocationProb'}\right)}
%		= \poly{\frac{\vol{\volume}}{\discretizationError \allocationProb}}
%	\]
%	such that for all $\numParticles \ge \volume$ it hold that a uniformly random $X \subset \volume$ with $\size{X} = \numPoints$ has a $\volumeError'$-$\distanceError'$-allocation with probability at least $1 - \allocationProb'$.
%
%	Setting
%	\[
%		\numPoints_{\discretizationError, \allocationProb} = \max\{128 \numTypes \fugacity_{\max}^2 \vol{\volume}^2 \discretizationError^{-1} \allocationProb^{-1}, \numPoints'_{\discretizationError, \allocationProb}\} \in \poly{\frac{\vol{\volume}}{\discretizationError \allocationProb}}
%	\]
%	now ensures that for all $\numPoints \ge \numPoints_{\discretizationError, \allocationProb}$
%	\[
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge \left(1 - \discretizationError'\right) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}
%	\]
%	with probability at least $1 - \allocationProb'$.
%	Further, \Cref{lemma:expectation} implies that
%	\[
%		\Pr{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} < \left(1 - \discretizationError'\right) \E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}}} \le \allocationProb'.
%	\]
%
%	By \Cref{lemma:modified_markov,lemma:expectation}, we obtain
%	\begin{align*}
%		\Pr{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge (1 + \discretizationError) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}}
%		&\le
%		\Pr{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge (1 + \discretizationError) \E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}}} \\
%		&= \Pr{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \ge (1 + c \discretizationError') \E{\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}}}} \\
%		&\le \frac{1}{c + 1} \left(1 + \frac{\allocationProb'}{\discretizationError'}\right) \\
%		&\le \frac{1}{c+1} \left(1 + \frac{1}{2}\right) \\
%		&\le \frac{3}{4} \allocationProb .
%	\end{align*}
%	Using the union bound on the failure probabilities, we obtain
%	\[
%		\left(1 - \discretizationError'\right) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity} \le
%		\hcPartitionFunction{\hcPPGraph{X}}{\hcPPWeight{X}} \le (1 + \discretizationError) \generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}
%	\]
%	with probability at least $1 - \allocationProb' - \frac{3}{4} \allocationProb = 1 - \frac{\discretizationError}{4} \allocationProb - \frac{3}{4} \allocationProb \ge 1 - \allocationProb$.
%	Finally, observing that $1 + \discretizationError \le \eulerE^{\discretizationError}$ and $1 - \discretizationError' = 1 - \frac{\allocationProb}{2} \discretizationError \ge \eulerE^{- \discretizationError}$ concludes the proof.
%\end{proof}
%
%\begin{remark}
%	Note that the concentration result without star-convexity, given in \Cref{thm:prob_bound_non_starconvex}, has a worse dependency on the desired error probability $\allocationProb$ than that obtained with star-convexity in \Cref{cor:random_discretization_concentration}.
%	This is due to the application of \Cref{lemma:modified_markov}.
%	However, the dependency is still sufficient to construct a fully polynomial randomized approximation scheme (FPRAS) for $\generalPartitionFunction{\volume}{\interactionMatrix}{\fugacity}$.
%\end{remark}
